A Resource-Efficient Decentralized Sequential Planner for Spatiotemporal Wildfire Mitigation

This paper proposes a Conflict-aware Resource-Efficient Decentralized Sequential planner (CREDS) for early wildfire mitigation using multiple heterogeneous Unmanned Aerial Vehicles (UAVs). Multi-UAV wildfire management scenarios are non-stationary, with spatially clustered dynamically spreading fires, potential pop-up fires, and partial observability due to limited UAV numbers and sensing range. The objective of CREDS is to detect and sequentially mitigate all growing fires as Single-UAV Tasks (SUT), minimizing biodiversity loss through rapid UAV intervention and promoting efficient resource utilization by avoiding complex multi-UAV coordination. CREDS employs a three-phased approach, beginning with fire detection using a search algorithm, followed by local trajectory generation using the auction-based Resource-Efficient Decentralized Sequential planner (REDS), incorporating the novel non-stationary cost function, the Deadline-Prioritized Mitigation Cost (DPMC). Finally, a conflict-aware consensus algorithm resolves conflicts to determine a global trajectory for spatiotemporal mitigation. The performance evaluation of the CREDS for partial and full observability conditions with both heterogeneous and homogeneous UAV teams for different fires-to-UAV ratios demonstrates a $100\%$ success rate for ratios up to $4$ and a high success rate for the critical ratio of $5$, outperforming baselines. Heterogeneous UAV teams outperform homogeneous teams in handling heterogeneous deadlines of SUT mitigation. CREDS exhibits scalability and $100\%$ convergence, demonstrating robustness against potential deadlock assignments, enhancing its success rate compared to the baseline approaches.

==> TexImages/test.tex <==
\begin{tikzpicture}[x=2.9in,y=2.9in]

\draw[help lines,xstep=.1,ystep=.1] (0,0) grid (1,1);
\foreach \x in {0,1,...,9} { \node [anchor=north] at (\x/10,0) {0.\x}; }
\foreach \y in {0,1,...,9} { \node [anchor=east] at (0,\y/10) {0.\y}; }


\draw[line width=0.25mm,dashed,] (0.0,0.02) -- (0.0+0.11,0.02);
\node[fill=white] at (0.27,0.025) {\small \shortstack[c]{Communication link}};
\draw[line width=0.25mm] (0.5,0.02) -- (0.5+0.11,0.02);
\node[fill=white] at (0.71,0.025) {\small \shortstack[c]{Power transfer}};

\draw[line width=0.25mm] (0.0,0.68) rectangle (0.8,0.6);
\draw[line width=0.25mm] (0.0,0.89) rectangle (0.8,0.81);
%\node[fill=white,inner sep=0.5ex] at (0.4,0.64) {\small \shortstack[c]{Community Microgrid Controller}};
\node[fill=white,inner sep=0.5ex] at (0.4,0.64) {\small \shortstack[c]{Central Controller}};
\node[fill=white,inner sep=0.5ex] at (0.39,0.845) {\small \shortstack[c]{Utility Grid }};
\draw[line width=0.25mm,dashed,to-to] (0.38,0.68) -- (0.38,0.81);
\draw[line width=0.25mm,to-to] (0.41,0.68) -- (0.41,0.81);
\node[fill=white, inner sep=0.3ex] at (0.18,0.75) {\small \shortstack[c]{ToU based tariff rate}};
\node[fill=white, inner sep=0.3ex] at (0.62,0.755) {\small \shortstack[c]{Total power exchange\\with UG}};

\node at (0.18,0.25) {\input{./TexImages/House_1.tex}};
\node at (0.6,0.25) {\input{./TexImages/House_2.tex}};
\draw[line width=0.75mm,dotted] (0.37+0.0,0.25) -- (0.42+0.0,0.25);
\node[fill=white] at (0.13,0.55) {\small Predicted power};
\node[fill=white] at (0.16,0.44) {\small \shortstack[c]{P2P sharing\\command}};
\draw[line width=0.25mm,dashed,to-to] (0.28,0.34) -- (0.28,0.6);
\draw[line width=0.25mm,to-to] (0.33,0.34) -- (0.33,0.6);
\draw[line width=0.25mm,dashed,to-to] (0.70,0.34) -- (0.70,0.6);
\draw[line width=0.25mm,to-to] (0.75,0.34) -- (0.75,0.6);
\node[fill=white, inner sep=0.3ex] at (0.49,0.45) {\small \shortstack[c]{Power exchange\\with CMC}};

\draw[line width=0.25mm,to-to] (0.2,0.14) |- (0.07,0.1);
\draw[line width=0.75mm,dotted] (0.06,0.1) -- (0.001,0.1);
\draw[line width=0.25mm,to-to]  (0.24,0.15) -- (0.24,0.1) -| (0.61,0.14);
\node[inner sep=0.2ex] at (0.4,0.15) {\small \shortstack[c]{P2P\\power transfer}};
\draw[line width=0.25mm,to-to] (0.65,0.145) |- (0.75,0.1);
\draw[line width=0.75mm,dotted] (0.755,0.1) -- (0.81,0.1);

\end{tikzpicture}
